Deterministic particle flows for constraining stochastic nonlinear systems

Devising optimal interventions for constraining stochastic systems is a challenging endeavour that has to confront the interplay between randomness and nonlinearity. Existing methods for identifying the necessary dynamical adjustments resort either to space discretising solutions of ensuing partial differential equations, or to iterative stochastic path sampling schemes. Yet, both approaches become computationally demanding for increasing system dimension. Here, we propose a generally applicable and practically feasible non-iterative methodology for obtaining optimal dynamical interventions for diffusive nonlinear systems. We estimate the necessary controls from an interacting particle approximation to the logarithmic gradient of two forward probability flows evolved following deterministic particle dynamics. Applied to several biologically inspired models, we show that our method provides the necessary optimal controls in settings with terminal-, transient-, or generalised collective-state constraints and arbitrary system dynamics.

==> notes.tex <==
Citations can be handled in one of three ways.  The most
straightforward (albeit labor-intensive) would be to hardwire your
citations into your \LaTeX\ source, as you would if you were using an
ordinary word processor.  Thus, your code might look something like
this:


\begin{quote}
\begin{verbatim}
However, this record of the solar nebula may have been
partly erased by the complex history of the meteorite
parent bodies, which includes collision-induced shock,
thermal metamorphism, and aqueous alteration
({\it 1, 2, 5--7\/}).
\end{verbatim}
\end{quote}


\noindent Compiled, the last two lines of the code above, of course, would give notecalls in {\it Science\/} style:

\begin{quote}
\ldots thermal metamorphism, and aqueous alteration ({\it 1, 2, 5--7\/}).
\end{quote}

Under the same logic, the author could set up his or her reference list as a simple enumeration,

\begin{quote}
\begin{verbatim}
{\bf References and Notes}

\begin{enumerate}
\item G. Gamow, {\it The Constitution of Atomic Nuclei
and Radioactivity\/} (Oxford Univ. Press, New York, 1931).
\item W. Heisenberg and W. Pauli, {\it Zeitschr.\ f.\ 
Physik\/} {\bf 56}, 1 (1929).
\end{enumerate}
\end{verbatim}
\end{quote}

\noindent yielding

\begin{quote}
{\bf References and Notes}

\begin{enumerate}
\item G. Gamow, {\it The Constitution of Atomic Nuclei and
Radioactivity\/} (Oxford Univ. Press, New York, 1931).
\item W. Heisenberg and W. Pauli, {\it Zeitschr.\ f.\ Physik} {\bf 56},
1 (1929).
\end{enumerate}
\end{quote}


That's not a solution that's likely to appeal to everyone, however ---
especially not to users of B{\small{IB}}\TeX\ \cite{inclme}.  If you
are a B{\small{IB}}\TeX\ user, we suggest that you use the
\texttt{Science.bst} bibliography style file and the
\texttt{scicite.sty} package, both of which are downloadable from our author help site.
{\bf While you can use B{\small{IB}}\TeX\ to generate the reference list, please don't submit 
your .bib and .bbl files; instead, paste the generated .bbl file into the .tex file, creating
 \texttt{\{thebibliography\}} environment.}
 You can also
generate your reference lists directly by using 
\texttt{\{thebibliography\}} at the end of your source document; here
again, you may find the \texttt{scicite.sty} file useful.

Whatever you use, be
very careful about how you set up your in-text reference calls and
notecalls.  In particular, observe the following requirements:

\begin{enumerate}
\item Please follow the style for references outlined at our author
  help site and embodied in recent issues of {\it Science}.  Each
  citation number should refer to a single reference; please do not
  concatenate several references under a single number.
\item The reference numbering  continues from the 
main text to the Supplementary Materials (e.g. this main 
text has references 1-3; the numbering of references in the 
Supplementary Materials should start with 4). 
\item Please cite your references and notes in text {\it only\/} using
  the standard \LaTeX\ \verb+\cite+ command, not another command
  driven by outside macros.
\item Please separate multiple citations within a single \verb+\cite+
  command using commas only; there should be {\it no space\/}
  between reference keynames.  That is, if you are citing two
  papers whose bibliography keys are \texttt{keyname1} and
  \texttt{keyname2}, the in-text cite should read
  \verb+\cite{keyname1,keyname2}+, {\it not\/}
  \verb+\cite{keyname1, keyname2}+.
\end{enumerate}

\noindent Failure to follow these guidelines could lead
to the omission of the references in an accepted paper when the source
file is translated to Word via HTML.





--------------
The challenge for evolution or bioengineers is to find sequences that exhibit some desired profile of functionalities y

dynamic landscape
seascape" fitness landscape that changes over time


in  lab,  we  can  increase  the  recombination  frequency,  i.e.ρ >>1andμ >>1/Lto generate farther diversity, as we get second attempts if a population ofmutants is completely dead.  On the critique side, they often bias and enhance theselective forceβtoward a particular phenotype of interest.  This is a double-edgedsword, on one hand this allows the power of evolution to be focused on a trait of interest, on the other hand it may result in deterioration of secondary traits that arealso important and multi-objective directed evolution is challenging



 KLD to quantify the dis-tance between equilibrium distributions of phenotypic traits
. Nourmohammad, S. Schiffels, and M. Lässig, Evolutionof molecular phenotypes under stabilizing selection


 if the KLDat this time is not too large, the B cell population evolvesin an attempt to adapt to the imposed selection force, re-sulting in reduction of the KLD with time.
 
 On average, the rate of decrease is slower (a) near optimal forcing [D(p0||f1)=3.15] and faster (b) beyond the optimum,D(p0||f1)=5.16.
 
 imposed selection force
 
 Molecular   phenotypes   are   important   links   between   genomicinformation   and   organismic   functions,   fitness,   and   evolution.   Complexphenotypes, which are also called quantitative traits, often depend on multiplegenomic loci. 
 
 covers evolutionary processes at high and low recombination rates,that is, it applies to sexual and asexual populations.
 
 We  derive  approximate  evolutionequations for the distribution of phenotype values within and across populations
 
 
 Many  such  phenotypes  arequantitative traits: they have a continuous spectrum of values and depend on multiplegenomic sites
 
 This calls for an effective
 
 
 
 
 
 
 
 ----
 Clonal populations stochasticallyswitch phenotypes in response to changes in the environ-ment. Recently, stochastic phenotype switching was directedtowards searching for optimal conditions that increase thefraction of generalists within a background population of bothspecialists and generalists
 
 
 The information regarding organism features is (partly) encoded in theirgenome, orgenotype. This dictates the expression of proteins in cells via tran-scription and translation that in turn build up thephenotypeof the organism.Actually phenotype is not entirely determined by genotype since there aremany sources of noise and errors when translating DNA into proteins andin the proteins function. Even knowing the exact genome of an organism it’svery hard to predict its phenotype, a problem known as genotype-phenotypemapping.  But in the context of evolution genotype is regarded as the mainentity  encoding  information  on  phenotype,  and  mutations  usually  denotechanges  in  the  genome,  also  because  only  those  changes  areheritableandpropagate through generations.
 Then natural selection acts on some collective traits arising from the phe-notype, and such traits largely depend on the environment and on the con-text in which selection acts.
 
  pheno-typic space and then defined a non-linear scalar function to map phenotypeto fitness 
  
  THE long-term evolutionary fate of a population relies on the shape of its adaptive landscape. The adaptive landscape is the precise map that associates a fitness value to any possible genotype or phenotype. 
  
  Fisher’s geometric model (Fisher 2000). Phenotypic fitness landscapes model how the genotype of an organism translates into a set of phenotypes, which themselves determine fitness. In other words, the very large space of all possible genotypes is projected onto a continuous phenotypic space of arbitrary dimensionality, and fitness depends only on the position in this phenotypic space. Fisher’s model, in particular, assumes that the phenotypes are under stabilizing selection toward a single optimum, that the effects of mutations in the phenotypic space are drawn from a multivariate Gaussian distribution, and that mutations combine additively in the phenotypic space. Phenotypes can be biological traits that need to be tuned to a precise level to maximize growth of the organism in the environment of selection, e.g., the concentration of an enzyme in a metabolic pathway or the level of expression of a gene. Fisher’s model also can be viewed as an abstract statistical description of the genotype fitness map.
  
   Fisher’s model emerges from a set of “first principles” that specifies how fitness results from developmental integration of a large number of mutable traits [Fisher’s geometrical model emerges as a property of complex integrated phenotypic networks. Genetics ]
   Last, Fisher’s geometric model is simple yet can generate a diversity of empirical landscapes (Blanquart et al. 2014), and it successfully predicts experimental quantities, such as the distribution of epistasis coefficient between pairs of mutations (Martin and Lenormand 2006; Martin et al. 2007) and the dynamics of mean fitness over time (perfeito et al. 2014).
   
       In Fisher’s model, individuals are characterized by a number of continuous phenotypes that are under stabilizing selection towards a single fitness peak in the multivariate phenotypic space. Mutations fuel the process of adaptation by generating new genotypes with different phenotypic values. One fundamental difference with the discrete models described above and phenotypic models is that in the latter, epistasis emerges from the non-linearity of the phenotype to fitness map, and not from random components.
    
    Epistasis refers to the existence of interactions between mutations: the effect of a mutation depends on the genetic background in which it appears. The spread of a mutation in a population depends on its effect on fitness and as epistasis affects fitness it can potentially influence the evolution of a population. This is why we focus here on the effect of mutations and their interactions on fitness.
    
    
    Epistasis is a key component of genomic architecture. Two main approaches, which can be traced back to the Wright vs. Fisher debate, have been used to study epistasis. In a Wrightian approach epistasis dominates the adaptive landscape such that the landscape is defined only by the epistatic interactions among mutations. Depending on the amount of epistasis and its (a priori imposed) distribution, smooth or rugged fitness landscapes can emerge (Goodnight 1988; Kauffman 1993; Hansen and Wagner 2001). The epistasis of the genotypes present in the population evolves then as the population wanders in such genetic space. In a Fisherian view (Fisher 1930), the adaptive landscape has a single peak, and epistasis either is included to modulate how fitness decays with the distance to the optimum (usually in terms of Hamming distance) or emerges as a consequence of the phenotype to fitness map (Wolf et al. 2000) 
    
     Fisher's model stipulates that organisms are characterized by a number of independent trait values. Each trait is under stabilizing selection, which means that a unique optimal value of the trait exists. This results in the existence of an optimal combination of traits that provides the best possible fitness (Figure 1A). 
     
     
     The number of independent traits, which in geometric terms is the number of dimensions of the space: We mention this parameter later as “the phenotypic complexity.”
     
     The way fitness declines for each trait given the distance to the optimal trait value: In this article, we use the same fitness decay function for all traits, which produces circular fitness isoclines. We decided to use a fitness function in which epistasis could be affected by a single parameter, Q. In agreement with previous studies, the function we use is f(x) = exp(−xQ) (Wilke 2001; Tenaillon et al. 2007), with x being the distance to the optimum and Q an epistasis parameter (see later).

The way mutations affect traits: In such a model a mutation is a vector that moves one organism defined by its position in the phenotypic space to a new position. In the present analysis the direction of the vector is drawn from a uniform distribution and its norm is drawn from a centered normal distribution with standard deviation equation M2.


Representation of Fisher's model in two dimensions. Here an organism is defined by a combination of its traits' x and y values; its fitness is a function of the distance of its phenotype (x1, x2) to the optimum genotype (0, 0), and therefore fitness isoclines are circular.


Selection gradient:
The selection differential is a coefficient often used to estimate selection but does not partition direct versus indirect selection, whereby direct selection results in phenotypic changes that are directly related to fitness whereas indirect selection can cause a phenotypic change that is not directly related to fitness because that trait is correlated with another trait that is under direct selection. The selection gradient was then introduced to quantify the direct relationship between a phenotypic trait and fitness and originally defined as the partial derivative of (relative) fitness with respect to the mean value for a phenotypic trait.
-------
variant of FGM, modified to incorporate arbitrary phenotypic correla-tions, provided good fits to DFE data from mutation accumulation experiments onmultiple organisms

 the assumptions that there is a single, stationary opti-mum are unlikely to be met in natural environments, which are both spatially andtemporally heterogeneous. These concerns have been addressed by incorporatinga moving optimum [51, 121, 196], genotype-by-environment interactions [51], andmultiple optima [195
 
 Phenotype-structured populations belong to the polymorphic category. In such populations, individuals are characterised by (typically) one quantitative trait which is related to reproductive success (fitness) [24]. A common way to model phenotype-structured populations is to describe the quantitative trait of interest by a continuous variable (although discrete versions are possible). Then, mutations are often described by diffusion operators acting on the space of phenotypes. Such properties allow the deterministic mutation-selection dynamics of the population to be described by means of integro-differential equations.
 
 
 
 
Here we consider the control of cell differentiation of a gene regulatory network. The considered controller is construed as a real-time \emph{in silico} feedback control\cite{del2016control} of the considered cell.  In silico control allows for manipulation of  dynamic behaviour of living cells without requiring permanent or genetic modifications of the living cell. Instead, the controller is implemented on a computer and the feedback is provided through one of the possible actuation methods.  In the rapidly expanding field of in silico controls, commonly employed state interventions 
are performed by means of optogenetic techniques~\cite{milias2011silico,toettcher2011light}, or through changes of osmotic pressure~\cite{uhlendorf2012long} or inducer concentrations~\cite{menolascina2014vivo}.

The reprogramming of cell fates is mediated through manipulation of the gene regulatory network that determines the phenotype of the cell. This reprogramming is typically implemented through overexpression of exogenous transcription factors. Transcriptor factors are DNA-binding proteins that determine how often genes are transcribed into messenger RNA (mRNA) for production of proteins. External presentation of transcription factors induce  trascriptional activation and inhibition directed through the cell's gene regulatory network.
Each one of the stable states in the dynamics of a gene regulatory network corresponds to one different cell phenotype. Cell fate decisions, i.e. transitions between different phenotypes, are often induced by external input or occur randomly due to noise \cite{wang2011quantifying}.
Although manipulation of transcription factors is often unreliable in \cite{del2016control} the authors propose a general purpose synthetic feedback controller that can drive the transcription factor contractions to any desired value.
%In particular, the controller implements feedback overexpression of each TF by concurrently realizing a large (inducible) production rate and a large degradation rate. The net result of these two large opposing forces is that the concentration of the TF approaches a well-defined “proportion” between the (synthetically realized) production and degradation rates, independently of the network that also regulates the TF.
%trigger state transitions in multistable gene regulatory networks in which preset overexpression fails.

%Major actuation methods include exposing the cell to light of a specific wavelength (optogenetics techniques) [116,118], changing osmotic pressure [117] or changing inducer concentration

Gene regulatory networks. We present our framework in a setting of triggering state transitions in a gene reguratory network.
We consider a set of coupled SDEs that capture the gene regulatory network's activity with $n$ transcription factors with concentrations denoted as $x_1, \dots, x_n$. Over-expression of transcription factors is expressed as external intervention $u_i$ that directly mediates the increase of production rate of transcription factor $x_i$.
The dynamical equation governing these dynamics may be written as
\begin{equation}
    dx_t^i = F(x_t^i) - \gamma_i x_t^i + u_t^i + \sigma dW_t
\end{equation}
where $F()$ denotes the Hill function capturing the regulatory interactions of the trascriptor factors, $\gamma$ denotes the constant decay rte due to dilution or degradation, and $u_i >= 0$. Here we have neglected the mRNA dynamics, assuming that mRNA quickly resorts to its quasi steady state.
The noise term captures all other processes, as well as transcription rate changes due to changing concentrations of
 transcription factor, and is assumed to be Gaussian white noise~\cite{ozbudak2002regulation}. 

We applied the proposed control framework to models of cell differentiation to induce lineage changes
\cite{corson2012geometry}
For the controlled numerical experiment with the Caenorhabditis elegans vulval precursor cell (VPC) differentiation model we employed the model

\begin{align}
    \frac{dx_1}{dt} &= \frac{x_1^4}{p_1^4 + x_1^4} + \frac{p_2^4}{p_2^4 + x_2^4} - x_1  + \xi_1(t)\\
     \frac{dx_2}{dt} &= \frac{x_2^4}{p_3^4 + x_2^4} + \frac{p_4^4}{p_4^4 + x_1^4} - x_2 + \xi_2(t),
\end{align}

with parameters $p_1 = p_2 = p_3 = p_4 = 0.5$ and independent Gaussian white noise sources $\xi_{\{1,2\}}$.


Since with current technologies the direct feedback control of individual cells is largely inaccessible, we considered two complementary scenarios for this setting. One when we assume hat direct state feedback control is feasible and we seek the optimal interventions in terms of state feedback, and one when we consider that only the system parameters are accessible to us, and therefore manipulate the system by computing the necessary parameter changes that will result in optimal state feedback control.

To that end, in the latter setting, we seek a perturbation in the system parameters $\alpha$ that will induce the necessary state feedback to drive the controlled system to the target state. More formally, we compute the necessary parameter changes $\delta \alpha_t$ that will render the following equality valid
\begin{equation}
f(X_t,t;\alpha + \delta \alpha_t) = f(X_t,t; \alpha) + u(X_t,t).
\end{equation}
Here we have explicitly denoted the dependence of the drift function $f(x,t;\alpha)$ on a set of parameters $\alpha$.
By employing a perturbation expansion to first order in $\delta \alpha_t$ in the left hand side
we obtain that the necessary parameter changes are
\begin{equation}
    \delta \alpha_t =  \left[\frac{\partial f}{\partial \alpha} \right]^{-1} u(x,t).
\end{equation}


We denote here that in this setting we compute the optimal state interventions and not the optimal parameter interventions.
In essence we minimise the term $ \int_0^T\| \frac{1}{2} u(x,t) H u^T(x,t) \|_2^2 dt$ instead of minimising
the terms 
\begin{equation}
\int_0^T\| \delta \alpha_t \cdot \delta \alpha_t^T \|_2^2 dt = \int_0^{\top} \| \left[\frac{\partial f}{\partial \alpha} \right]^{-1} u(x,t) \cdot u^T(x,t) \left[\frac{\partial f}{\partial \alpha} \right]^{-\top} \|_2^2  dt. 
\end{equation}
These two terms are minimised at the same time when $f(x,t;\alpha)$ is linear in $\alpha$.

For a more general drift with nonlinear dependence on the parameters $\alpha$, the optimal state interventions in terms of $u$ do not necessarily reflect optimal parameters interventions. 
Moreover, since we have assumed that $H \propto \sigma^{-1}$ to linearise the Hamilton-Jacobi-Bellman equation, under the current assumptions, this formalism might not be adaptable for identifying optimal parameter interventions. However, we leave this issue for future research.

\textcolor{magenta}{ in silico feedback control where the controller is implemented in the computer and implements controls by modifying nutrintient concentratoins necessary for cell fucntionn - is not constrained by the genetic nature/biochemical processes ingrained in the cell of living cells like in-cell control, and arbitrary controllers may be implemented; control mediated through exposing the cell to light of a specific wavelength (optogenetics techniques)  changing osmotic pressure  or changing inducer concentration~\cite{del2016control}}
%\textcolor{magenta}{E.Science is better now a] our strength b] what it is useful for}

In practice, we require to compute the difference between the two gradient log densities, $p^*(x,t)$ and $\rho(x,t)$, capturing the densities of the forward and marginal densities. To compute these,we propagate forward in time from $t=0$ to $t-T$ the probability flow of $\rho(x,t)$ according to Eq.(\ref{FPE2}) starting from $x = x_0$. At every timestep of the forward propagation, we reweight the particles according to the deterministic optimal transport reweighting algorithm. This gives a representation of the forward density. As a second step, starting from the target state $x^*$ at time $T$ we sample backwards in time the density $p^*(x,t)$
simulating the probability flow dynamics of Eq.(\ref{eq:controlled_dyn}-\ref{backward_drift}).
This requires the computation of $\nabla \ln \rho(x,t)$ at each time point. To that end, our sampling scheme involves a forward simulation of the free dynamics (Eq.()), followed by a backward simulation of the dynamics ... that create samples from the required marginal density.
We represent probability densities with particles, and employ the probability flow deterministic dynamics to evolve the densities in time.

\textcolor{magenta}{
 Although direct in-vivo state manipulations of single cells are largely inaccessible with the present technology, we have construed the control as a real-time \emph{in silico} feedback control\cite{del2016control} of the considered cell.  In silico control allows for manipulation of  dynamic behaviour of living cells without requiring permanent or genetic modifications of the living cell. Instead the controller is implemented on the computer and the feedback is provided through one of the possible actuation methods. In the rapidly expanding field of in silico controls, commonly employed state interventions 
are performed by means of optogenetic techniques~\cite{milias2011silico,toettcher2011light}, or through changes of osmotic pressure~\cite{uhlendorf2012long} or inducer concentrations~\cite{menolascina2014vivo}.
However as detailed in the appendix we have additionally modified our framework to derive necessary parameter adjustments from the optimal state perturbation to imitate thereby manipulation with current in-vivo techniques.
To reprogram cell fate manipulation of the gene regulatory network that determines the cell's phenotype. This reprogramming often is implemented through manipulation/overexpression of transcription factors, although this method is unreliable and not deterministic. 
Although manipulation of transcription factors is often unreliable in \cite{del2016control} the authors propose a general purpose synthetic feedback controller that can drive the transcription factor concentrations to any desired value.
In particular, the controller implements feedback overexpression of each TF by concurrently realizing a large (inducible) production rate and a large degradation rate. The net result of these two large opposing forces is that the concentration of the TF approaches a well-defined “proportion” between the (synthetically realized) production and degradation rates, independently of the network that also regulates the Transcription Factor.
trigger state transitions in multistable gene regulatory networks in which preset overexpression fails.
Major actuation methods include exposing the cell to light of a specific wavelength (optogenetics techniques) [116,118], changing osmotic pressure [117] or changing inducer concentration
}


In practical scenarios, direct manipulation of cell state is generally experimentally inaccessible. 


in  lab,  we  can  increase  the  recombination  frequency,  i.e.ρ >>1andμ >>1/Lto generate farther diversity, as we get second attempts if a population ofmutants is completely dead.  On the critique side, they often bias and enhance the selective forceβtoward a particular phenotype of interest.  This is a double-edgedsword, on one hand this allows the power of evolution to be focused on a trait of interest, on the other hand it may result in deterioration of secondary traits that arealso important and multi-objective directed evolution is challenging
problematic simplifying assumptions that many fitness landscape models make
(such as a fixed environment).
----

I think we need the adjoint instead of the time reversed.

The adjoint changes sign only on the irreversible dynamics  [https://iopscience.iop.org/article/10.1088/1742-5468/2006/08/P08001/pdf]
and this has zero entropy production [https://journals.aps.org/prresearch/pdf/10.1103/PhysRevResearch.3.L042012 ], while the time reversed changes sign on the entire drift vector and this under non-equilibrium conditions i.e. in nonconservative systems, for which we intrduced the algo 2 results in non zero KL divergence between forward and time reversed process .

Adjoint dynamics are constructed from
normal dynamics in order to preserve a stationary pdf pst but to
reverse the probability current. 

How to construnct adjoint: https://journals.aps.org/pre/pdf/10.1103/PhysRevE.92.042108

In essence you need to substract the grad log of the stationary density i.e the reversible part and reverse sign  ( $-f(x) + \sigma^2 \nabla \ln p_{st}(x)$ ).
Analytic derivation of stationary or long simulation?

But is the stationary density of the controlled dynamics, but control term s already a "potential term" thus reversible so doesnt matter?



Do I need decomposition in irreversible and reversible or is there any other way to obtain stationary, except from long simulations?


ow to construct https://journals.aps.org/pre/pdf/10.1103/PhysRevE.87.062109

Test the example 



This one seems to give the comparison
https://iopscience.iop.org/article/10.1088/1742-5468/2006/08/P08001/pdf
Eq.14 - same dynamics with time reversed current require $-f(x)+ \nabla \ln p^{st}(x)$ probably a sigma square missing
